On the origin of polar planets around single stars

The Rossiter-McLaughlin effect measures the misalignment between a planet's orbital plane and its host star's rotation plane. Around 10$\%$ of planets exhibit misalignments in the approximate range $80 - 125^\circ$, with their origin remaining a mystery. On the other hand, large misalignments may be common in eccentric circumbinary systems due to misaligned discs undergoing polar alignment. If the binary subsequently merges, a polar circumbinary disc -- along with any planets that form within it -- may remain inclined near 90$^{\circ}$ to the merged star's rotation. To test this hypothesis, we present $N$-body simulations of the evolution of a polar circumbinary debris disc comprised of test particles around an eccentric binary during a binary merger that is induced by tidal dissipation. After the merger, the disc particles remain on near-polar orbits. Interaction of the binary with the polar-aligned gas disc may be required to bring the binary to the small separations that trigger the merger by tides. Our findings imply that planets forming in discs that are polar-aligned to the orbit of a high-eccentricity binary may, following the merger of the binary, provide a possible origin for the population of near-polar planets around single stars.

==> Response.tex <==
We thank the referee for the useful report that has helped us to improve the manuscript. We have thoroughly reviewed the referee’s comments and made several changes to the manuscript. Referee-prompted changes in the updated document are highlighted in bold text. Additional edits, clarifying our methodology and results, are included, but not highlighted. We hope that you are satisfied with the revised manuscript.
Sincerely,
Cheng Chen, Stanley A. Baronett, C. J. Nixon & Rebecca G. Martin

Appended below are the referee comments immediately followed by our responses:


Assistant Editor's Comments:

The title added during the submission process on the Monthly Notices ScholarOne website differs slightly from the title on your manuscript. Could you please correct this when submitting your revised manuscript.

RESPONSE: We have corrected the title of our revised manuscript.


Scientific Editor's Comments:

Comments to the Author:
The detailed comments provided by the reviewer in the attached report cast doubts on the relevance of the proposed scenario for the origin of planets on polar orbits. This has therefore an impact on the level of urgency of the communication. The authors are invited to address in detail all the points and constructive criticisms contained in the reviewer's report when preparing a substantially revised submission. As the changes will likely have an impact on the overall paper length, I am ready to consider the revised manuscript for publication in the Main Journal.

RESPONSE: We request that you continue to consider the manuscript for publication in MNRAS Letters please. We have addressed the comments from the referee in detail while continuing to satisfy the length requirements of a letter. We present a novel method for generating planets on polar orbits around single stars. This method has not been discussed or proposed in the literature. We therefore do not agree with the referee that an exhaustive investigation is required at this stage (but we included two additional simulations to show that the binary can merge in more general parameters). We would like to quickly communicate the idea to the wider community -- we believe this is best done through publication of the idea, alongside a proof-of-principle calculation, in a Letters journal. We plan to address the details in subsequent papers. The referee has concluded that our mechanism is "possible". We agree that it is unclear at this stage whether this mechanism produces some, all or none of the observed polar planets around single stars -- we have not claimed to answer this question here. To do so would required detailed population synthesis that is beyond the scope of our current submission. This topic is an active field, on both the observational and theoretical sides, and we hope this paper will stimulate both theorists and observers to explore the scenario we propose.

Reviewer's Comments:
Reviewer: 1

Comments to the Author
This article present an interesting scenario to account for the recent detection of polar planets around single stars. The introduction is complete and presents the current open questions in the field and motivates the presented study. There are however a number of important shortcomings that prevent me for recommending this article for publication in the present form. The most critical one is that all the conclusions drawn by the authors rely on a single N-body simulation with very specific initial conditions (compact binary with a=0.1 au, m1=m2 and e=0.8). This mechanism is therefore possible, but it is unclear if it is relevant at the general level to account for the observed polar planets around single stars. Hence, a more detailed and thorough analysis is required to motivate its relevance.

RESPONSE: In the discussion section of the paper we now include two additional simulations for a different binary eccentricity and binary mass ratio. We show the final inclination of the circumbinary particles and see that they are close to polar after the binary has merged. We have therefore increased the range of binary parameters and find similar results. 

Below you will find a detailed list of comments and suggestions. After revising the article, I would recommend the authors to submit it as a standard publication in MNRAS.

ABSTRACT:
- "simulations": the authors should mention that a single simulation is done in this work, explicitly.
- "debris disc": the authors should clarify that this disc is not modelled in this work or that it is modelled as a (massless) test particle (no proper disc is considered in Section 3).

RESPONSE: We have clarified the text and note that we now present more than one simulation in the manuscript as the referee requested.


INTRODUCTION:
- It would be relevant to cite the recent works by Ceppi+(2023,2024) when talking about highly misaligned discs/planets in binary (or multiple) star systems. Some of their statistical trends could also be discussed later in the article.

RESPONSE: We have added these references in the Introduction and the Discussion. 


SIMULATION SETUP AND RESULTS
- WHFAST is an efficient and fast integrator but, in some cases, it leads to large errors if not handed properly. Have the authors tested more accurate integrators such as ias15? For computational costs, this could be acceptable for a paper presenting thousands of calculations. In this case, with a single calculation, I would recommend testing different integrators to make sure that the dynamics do not depend on the integrator choice.

RESPONSE: Given the dynamics present in these simulations the WHFAST integrator is adequate. To confirm this we re-ran all the simulations with IAS15 as well. We find the results are unchanged. As IAS15 is, in principle, more accurate, we now present those results in the paper.   

- The authors argue that the inner binary could shrink due to angular momentum exchange with the outer disc (not modelled here). In that case the disc should be fairly massive, which seems in tension with the scenario considered in this work (debris disc in the abstract). How massive should the disc be to effectively cause the necessary binary shrinking which then lead to tidal friction forces at the binary level? Does this happen in star formation regions? This aspect should be addressed in more detail to motivate the starting point of this scenario. Otherwise, the initial condition seems somewhat unrealistic and specifically chosen to lead to the binary merge scenario.

RESPONSE:
The disc mass by itself does not determine whether a binary can be brought to merger as, in principle, a disc of any non-zero mass can merge a binary. This is because the binary can continue to transfer angular momentum to the disc which can be carried away to large radius (see, for example, Pringle 1991). We are not sure where the referee infers that we are talking about interaction with a polar aligned debris disc to generate the binary shrinkage, as we state explicitly (in the abstract and main body of the paper) that we are discussing polar aligned gas discs in this regard, which have been shown to reduce the binary separation over time (Aly et al. 2015; Martin & Lubow 2019). Mergers of some protostars in star forming regions are generally thought to occur (e.g. Bally, 2005) and also for main-sequence stars (e.g. Wang, Langer et al. 2022). Providing a detailed population synthesis of merging binaries is beyond the scope of this initial letter which outlines a new idea for the formation of polar planets around single stars.


- After binary shrinking due to angular momentum exchange with the disc, does the disc inner edge remain at a fixed location or does it shrink together with the binary? This should be mentioned explicitly to motivate the inner edge at 3 a_b.

RESPONSE: As the referee has noted, our simulations employ a disc comprised of test particles. Thus, in our simulations, the binary does not shrink due to interaction with the disc.

- As in most literature, I would recommend using the gravitational constant G instead of k^2.

RESPONSE: We have replaced K^2 with G in the equation 1 and text.


DISCUSSION
- The binary interaction with a circumbinary disc is mentioned here. The authors should give more details about the expected fraction of binaries with discs that should eventually merge. The physics is well explained, but shrinking timescales are missing for binaries with surrounding protoplanetary discs. For instance, if this mechanism is relevant, should we expect some of the known binaries with (aligned/misaligned) discs to merge eventually? The decay rate is so fast in the only simulation presented that the binary shrinks in about 1000 orbital periods (a few thousand days). Is this observed in the known field binaries with separations of the order of 0.1 au and high eccentricities? This aspect should be discussed in the context of the available observations.

RESPONSE: In this letter we do not seek to provide an answer to the disc-binary interaction problem. The rate at which a circumbinary disc leads to binary orbital evolution is an open and active question in the field. However, looking at the observed distribution of stellar binaries (see, e.g., Fig. 14 of Raghavan et al. 2010) at periods of around 10 days and less (corresponding to semi-major axes of order 0.1 au and less) there is a noticeable lack of high eccentricity systems. This may well be due to the merger of these systems. We have discussed this point in the the 4th paragraph of Sec. 3.


- The recent works by Muñoz et al. should be discussed in this context, as these authors suggest that in some cases the binary semi-major axis could actually grow. Could this also happen in the scenario considered here?
	
RESPONSE: We have already referred to these works. Further we have noted that existing studies in the literature with polar aligned discs find that, as assumed here, the binary shrinks with time. 


- "We can therefore expect that in some regions of parameter space ...": this statement is too generic and vague/speculative. The authors should be more quantitative here.

RESPONSE: We have added additional detail to this comment.


- The work by Cuello & Giuppone (2019) considered the scenario in which a single circumbinary planet (decoupled from the disc) inherits the high tilt of the disc. In that case, the inner binary (besides potentially becoming more eccentric as mentioned by the authors) can start precessing as well. This should be mentioned here.

RESPONSE: We have included a reference to this paper.

- At a more general level, is it possible to (theoretically) compare the fraction of expected polar planets in binaries with the fraction of expected polar planet in singles (after merger)? This should strongly depend on the orbital parameters. I would appreciate if the authors could comment on this.

RESPONSE: To answer this question would require a more detailed understanding of planet formation and subsequent migration than is currently available in the literature. It would also depend, as the referee notes, on the binary orbital properties, and also on the stability properties of the systems that are formed. To compare with observations, we would also have to account for the other mechanisms that have been proposed to form polar planets around single or binary stars. For these reasons we prefer not to speculate on the outcome here and defer a detailed calculation to future work. The formation of planets around binaries is an interesting topic that is yet to be fully understood.

 
CONCLUSION
- "a combination of effects that likely include ...": the authors should rephrase this sentence since no statistical calculations are done in this article. This is not proved here as only one simulation is presented. At the moment, it sound a bit too speculative.

RESPONSE: We have reworded the sentence.


==> Response2.tex <==
We thank the new referee for the useful report that has helped us to improve the manuscript. We have thoroughly reviewed the referee’s comments and made several changes to the manuscript. Referee-prompted changes in the updated document are highlighted in bold text. Additional edits, clarifying our methodology and results, are included, but not highlighted. We hope that you are satisfied with the revised manuscript.
Sincerely,
Cheng Chen, Stanley A. Baronett, C. J. Nixon & Rebecca G. Martin


This manuscript posits an interesting new method to generate planets on highly misaligned orbits around single stars. The authors propose that these stars may have originally been eccentric binaries surrounded by a disc which was promoted to a polar aligned orbit. This binary then merges due to tidal interactions, leaving a planet on a strongly misaligned orbit around a single star. The purpose of this Letter is to test if a disc of test particles that is originally polar will remain so during the merger process. It does not address the tidal shrinking of the binary through disc interactions nor does it include any gas effects, it relies on N-body calculations only. I have independently assessed the manuscript and considered the previous referee report and reply in turn.

I agree with the authors that a population synthesis study or thorough parameter sweep is not within the scope or design of the paper. However, even with the simulations added in response to the first report the idea presented here is still incomplete. Of particular concern is the parameters used for the simulations that are chosen to prove this concept, where the binary has an orbital period of 8.166 days and an eccentricity of 0.8.

These parameters are chosen to demonstrate the effect but they are not typical of these systems: a high eccentricity is crucial to the polar alignment of these discs but as stated in the manuscript ‘Binaries with orbital period less than 12 days are close to circular’. (I note that in their reply the authors suggest this trend may well be due to the merger of these systems but provide no evidence that this is the case, it is speculation). This suggests that binaries with a small semi-major axis but a large eccentricity are quite unlikely, yet this is exactly what is needed in their simulation. This concern has been raised by the first referee and the authors have dutifully added two simulations in an attempt to address this. However, these simulations consider an eccentricity of 0.65 and a mass ratio of 1/3 – neither of these has moved the simulation out of the contrived parameter space.

To address this concern shared by myself and the first referee I recommend conducting at least two new simulations. I suggest one with a genuinely low eccentricity (e=0.2 or less) and one with a larger semi-major axis. Showing that planetesimals remain strongly misaligned under these circumstances would genuinely demonstrate that this is a viable method to make misaligned planets rather than a consequence of carefully chosen initial conditions. I understand the authors desire to publish this result quickly and thus have kept their previous corrections within the length requirements for a Letter. To retain this the authors could remove the simulations with e=0.65 and q=1/3 and replace them with the suggested simulations. They could also retain them all and consider resubmission to the main journal. 

RESPONSE: The main reason for the selected initial conditions of our fiducial model is to provide a simple model to demonstrate this process. On the other hand, to trigger the binary merger, e_b and a_b do not need to be so contrived. To address this, we followed the referee's advice and provided two new models. First, we consider a model with e_b =0.2, and second we consider a the model with a_b = 0.2 au (T_b = 32.25 days). In these two models, the mergers occur in 130,000 yrs and 11,000 yrs, respectively while their discs are still near polar. For a main sequence binary with e_b < 0.2, we expect it will take much longer to merge than the other models unless the binary separation is smaller. Hence, we mentioned the results of Raghavan et al. (2010) to indicate that there is a lack of binaries with semi-major axes of order 0.1 au (or less) and eccentricities greater than 0.1. 

However, we do not take  binary-disc interactions into account, which in principle shrinks the binary separation with time. Thus, the main goal of this paper is to address this mechanism to form a misaligned planet around a single star via the binary merger. In a following study, we will explore the shrinkage rate of the binary with the polar disc-binary interaction. As the eccentric binary system shrinks, tidal forces will take over the evolution of the binary. Hence, we feel the exploration of a wide range of parameter space in this study is not necessary.


In addition to this they must clarify the following points:
Timescales: In Section 2 it is stated that the binary orbital period must be less than 20 days to achieve merging within `a reasonable timescale’ but this statement is not justified. What sets the reasonableness of the timescale here? As it stands, it appears that the timescale for merging must be comparable to or larger than the timescale for the disc to align to polar (e.g. Aly et al. 2015). Explain if this is indeed the case and quantify what is meant by ‘reasonable’.

RESPONSE: We thank the referee for mentioning this. We have added the lower limit on the timescale of the polar alignment timescale of the gas disc. In addition, there is an upper limit on the timescale. From figure 14 in (Raghavan2010), we know that main sequence binaries have a moderate e_b distribution for orbital period T_b > 30 days and and a wide range of e_b for T_b > 100 days, implying the tidal dissipation between two solar-type stars with T_b > 30 days is too weak to trigger a merger. We have deleted the "reasonable timescale" and added some sentences to make our point clearer.

Section 2: Explain why the angle i=180 is chosen and plotted on Figure 2. Additionally it is stated that ‘If |i_s| in Equation 1 is larger than 1.0, i cannot be excited by this excitation’. Justify why the limit as written here is |i_s| > 1.0.

RESPONSE: Thank you for pointing out this typo. We meant to write that if cos(i_s) > 1.0 (i.e. the right hand side of equation 1), a particle should undergo the other type of the precession to the binary (nodal circulation) which means i_p will remain fixed with time (see the lower-right panel of the figure 2 in Lepp et al. 2022). We have added some text to describe this. 

Section 3: There appears to be confusion here with regards to the test particles being affected by tides. Here the manuscript states that the results remain similar whether or not GR effects are included because ‘the precession timescale of GR is much longer than that for tidal interactions’ which implies the particles are affected by tides (as this is more important than GR). However new text in Section 2 states that the particles are ‘not subject to tides’. Clarify.

RESPONSE: We thank the referee for pointing this out. The precession mentioned in the first paragraph of Section 3 refers to the apsidal precession of the binary's orbit (which can be due to tides or GR), and not to the test particles. We have clarified this in the text.
